When Eye-Tracking Meets Machine Learning: A Systematic Review on Applications in Medical Image Analysis

Eye-gaze tracking research offers significant promise in enhancing various healthcare-related tasks, above all in medical image analysis and interpretation. Eye tracking, a technology that monitors and records the movement of the eyes, provides valuable insights into human visual attention patterns. This technology can transform how healthcare professionals and medical specialists engage with and analyze diagnostic images, offering a more insightful and efficient approach to medical diagnostics. Hence, extracting meaningful features and insights from medical images by leveraging eye-gaze data improves our understanding of how radiologists and other medical experts monitor, interpret, and understand images for diagnostic purposes. Eye-tracking data, with intricate human visual attention patterns embedded, provides a bridge to integrating artificial intelligence (AI) development and human cognition. This integration allows novel methods to incorporate domain knowledge into machine learning (ML) and deep learning (DL) approaches to enhance their alignment with human-like perception and decision-making. Moreover, extensive collections of eye-tracking data have also enabled novel ML/DL methods to analyze human visual patterns, paving the way to a better understanding of human vision, attention, and cognition. This systematic review investigates eye-gaze tracking applications and methodologies for enhancing ML/DL algorithms for medical image analysis in depth.

==> Steps.tex <==
 run an
experiment to investigate if artificial intelligence (AI) can
assist in detecting radiologists’ gaze patterns that correlate with fatigue. 

We have demonstrated that deep-learning-based segmentation
of anatomical structures on medical images, in our case segmentation of lung fields from chest X-rays, can be extended further
than classical computer-aided diagnosis applications.


: There wasnt many paper related to neuroscince in the review paper, I belive this would the result of the phd.: Also summarizes the advances in ML/DL-based analysis methods for the analysis of eye-tracking data in neuroscience research.

==> Tips_from_papers.tex <==
1.  Visual acuity is highest at the \textbf{fovea}, a central region of the retina(Cowey and Rolls 1974). The foveal region has the highest density of photoreceptors that allows parts of the visual field that fall on it to be seen with the highest detail (Curcio et al. 1990).

2.  \textbf{saccades }that just move the eyes from target to target, smooth pursuit that allow tracking moving objects, reflexive eye movements that stabilize vision, and vergence eye movements that coordinate the two eyes to allow binocular fixation at different depths. In 
Vision is typically blurred during a saccade which allows for manipulation of the visual scene to go largely unnoticed during the saccadic interval.

3.  The eye tracking methods used to register eye movement to find the direction and targets of a person’s gaze are well in line with the nature of the topic. Such information is useful not only in revealing abnormalities in eye functioning and thus ensuring appropriate therapy but also in cognitive studies focused on learning about peoples’ emotions, intentions and how
they utilize their knowledge and skills. 

4. eye movement visualization, which relates gazes to areas of an observed scene and facilitates understanding analyzed processes.  

5. eye tracking methods and algorithms, as well as the eye movement characteristic were explained...
6. Eye-tracking technology has been used within a multitude of disciplines to provide data linking eye movements to visual processing of various stimuli (i.e., x-rays, situational positioning, printed information, and warnings)

7*** Over the past decade, deep learning has achieved unprecedented successes in a diversity of application domains, given large-scale datasets. However, particular domains, such as healthcare, inherently suffer from data paucity and imbalance.

8* Human eyes represent a rich source of information, for communicating emotional and mental conditions, as well as for understanding the functioning of our cognitive system. An eye gaze can serve as an appropriate proxy for learning a user’s attention or focus on context [1]. Therefore, eye-tracking technology has been intensively utilized for studying and analyzing many aspects of gaze behavior.

9.In eye tracking research, a fixation is indeed defined as a period during which the eyes remain relatively still and focused on a specific point or object. Fixations are characterized by a cluster of closely spaced gaze points, indicating that the person's gaze is locked onto a particular area or object of interest.
10. if a series of gaze points is very close – in time and / or space – this gaze cluster constitutes a fixation, denoting a period where the eyes are locked towards an object.

11.Eye tracking has emerged as a powerful tool for several applications, including health assessment and intervention, and human behavior and communication analysis.

\subsection{from }
12.Gaze tracking consists of the procedure of obtaining the direction or the point of regard (PoR) of the gaze with continuity, on a digital screen or in the physical environment, and it is achieved through mechanical, electronic, optical, and/or other methods.

13.Although researchers often use the terms of eye tracking and gaze tracking as synonyms, there is a slight difference between them. In particular, eye tracking is the measurement of eye movement/activity, while gaze tracking is the analysis of eye tracking data with regards to the head or the visual scene

14. In other words, eye tracking consists in detecting the existence and position of the eyes into an image and to track them over time (in the following images), and then in measuring activities as eye blinks, fixations, saccadic movements [15], pupil dilation [16], etc. The term gaze tracking instead refers to the estimation (and the temporal tracking) of where a person is looking at.

15.there are different ways to refer to the problem of estimating the human gaze from images: eye detection, eye tracking, eye localization, gaze estimation, gaze tracking, and point of regard are often used almost interchangeably and this can, sometimes, confuse the reader and hinder focusing the actual problem.

16.However, in the last 20 years, computer vision and machine learning have made progress from a methodological point of view and, at the same time, optical sensors have become increasingly advanced (high spatial and temporal definitions) and cheap. This encouraged researchers to make the effort to automatically extract knowledge from visible light images moving, this way, systems complexity from the hardware to the software side.


17.Eye tracking and gaze estimation are essentially two areas of research

==> use_for_writting.tex <==
\subsection{Eye-gaze Tracking Data in Medical Imaging} 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Eye-gaze Tracking and Medical Expert Analysis}

S-001: Around 60-80percent  of radiological errors are attributed to overlooked abnormalities, their research problem:"to investigate if artificial intelligence (AI) can
assist in detecting radiologists’ gaze patterns that correlate with fatigue?" and they tested implemented four fatigue/concentration measurement tests.
SE-002: talked about the radiologist error.


 S-004:Here's why Classification is the most relevant task:
Core Focus of the Research: The primary objective of the study is to classify expertise levels based on eye movement patterns. The DeepScan method is specifically designed to distinguish between experts and novices by analyzing their gaze behavior.
Alignment with Deep Learning Techniques: The use of the VGG-16 CNN architecture in the research is typically associated with classification tasks in machine learning. CNNs are highly effective in image-based classification, which is a central element of the study's methodology.
Applicability in Training and Evaluation: In the context of training and educational applications, classification plays a crucial role. Being able to classify a trainee's level of expertise accurately can help tailor the training content and methods to their specific needs.
Direct Measurement of Study Goals: The effectiveness of the DeepScan method is measured by its ability to accurately classify eye movement patterns, which directly correlates with the success of the research objectives.
While tasks like localization, segmentation, and data annotation are important in various contexts of machine learning and eye-tracking studies, the classification task aligns most closely with the goals, methods, and findings of this particular research.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

2.3 Eye-gaze Tracking Tasks

s-005:"The way humans attend to, process and classify a given image has the potential to
vastly benefit the performance of deep learning models. Exploiting where humans are
focusing can rectify models when they are deviating from essential features for correct
decisions. To validate that human attention contains valuable information for decisionmaking processes such as fine-grained classification, we compare human attention and
model explanations in discovering important features."



Classification, Localization, and Segmentation: These tasks are more directly related to the processing and interpretation of the medical images themselves (e.g., identifying areas of interest, classifying types of lesions, etc.),

for data annotation:about understanding the process and patterns of how radiologists view and interpret these images, rather than the images themselves.

for "detection to diagnosis":"Enhanced Interpretability and Reliability: By focusing on where and how intensively radiologists look at CXR images, the research contributes to a deeper understanding of diagnostic processes. This aligns well with disease detection and classification, where interpretability is crucial for clinical decision-making and justifying AI-based recommendations.
Application in Automated Diagnostics: The methodology developed in the paper could be pivotal in creating more accurate and reliable AI systems for automated disease detection, diagnosis, and classification in CXRs. It offers a step forward in bridging the gap between automated systems and human experts in radiology."


maybe can use this for writting:"Alignment with Study Goals: The primary goal of the study is to differentiate between radiologists of varying levels of expertise based on their eye-tracking data. Classification perfectly aligns with this objective, as it involves categorizing data into predefined classes—in this case, differentiating between faculty and trainee radiologists.
Utilization of Machine Learning: The study heavily employs machine learning classifiers, such as Gaussian process, Logistic regression, K-nearest neighbors, XG-Boost, and a modified AlexNet. These classifiers are fundamentally designed for classification tasks, making it the most relevant task for the methods used in the paper.
Data Analysis Suitability: The discretized feature encoding of fixation data created in the study is ideal for a classification approach. The method involves analyzing and categorizing eye movement patterns, which is inherently a classification task.
Performance Metrics Compatibility: The performance metrics used in the study, such as Area Under the Curve (AUC), Accuracy, F1 Score, Sensitivity, and Specificity, are typically used to evaluate the effectiveness of classification models.
Direct Impact on Research Problem: Classification directly addresses the research problem of perceptual errors in radiology by enabling the identification of different levels of diagnostic expertise, which can inform training and improvement strategies."








For localization:"Focus on Radiologist's Gaze: The paper emphasizes understanding where radiologists look when diagnosing chest X-rays (CXR). This aligns closely with the task of localization, which involves identifying specific areas or features within an image. The proposed system aims to not only locate where radiologists focus their attention but also to understand the intensity of this focus, which is a critical aspect of localization.
Enhanced Interpretability through Localization: By localizing the areas of interest in CXR images, as determined by the radiologists' gaze, the research contributes to developing AI systems that are more interpretable. This is because localization can provide clear visual evidence of why certain areas are significant for diagnosis, which is in line with the paper's goal of creating interpretable AI systems.
Direct Relevance to Diagnostic Processes: In medical imaging, especially in CXR analysis, localization is crucial for identifying pathological features. The approach of this paper to use radiologists' gaze intensity for localization directly contributes to improving the accuracy and reliability of diagnostic processes in radiology."








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Eye-gaze Tracking Applications


based on the s-009:Choosing between these applications would depend on various factors such as the specific needs of the healthcare facility,




based on S-002:the primary objective of radiology—accurate disease detection and diagnosis. Improvements in this area can lead to earlier and more precise identification of conditions like cancer, which is crucial for patient outcomes.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Eye-gaze Tracking Methods}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Visual attention learning / visual search pattern/ saliency methods

SE-002,
S-007

the use of visual maps to illustrate differences in search patterns between subjects






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
2.7 Evaluation Metrics/Performance Experiments
